Solar Wind Helium Abundance Heralds Solar Cycle Onset

We study the solar wind helium-to-hydrogen abundance's ($A_\mathrm{He}$) relationship to solar cycle onset. Using OMNI/Lo data, we show that $A_\mathrm{He}$ increases prior to sunspot number (SSN) minima. We also identify a rapid depletion and recovery in $A_\mathrm{He}$ that occurs directly prior to cycle onset. This $A_\mathrm{He}$ Shutoff happens at approximately the same time across solar wind speeds ($v_\mathrm{sw}$), implying that it is formed by a mechanism distinct from the one that drives $A_\mathrm{He}$'s solar cycle scale variation and $v_\mathrm{sw}$-dependent phase offset with respect to SSN. The time between successive $A_\mathrm{He}$ shutoffs is typically on the order of the corresponding solar cycle length. Using Brightpoint (BP) measurements to provide context, we infer that this shutoff is likely related to the overlap of adjacent solar cycles and the equatorial flux cancelation of the older, extended solar cycle during Solar Minima.

==> SOLA_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{{\it et al.}}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})



==> latex-preamble/abbreviations.tex <==
\acro{AR}{active region}

\acro{CDAweb}{Coordinated Data Analysis Web}
\acro{CH}{coronal hole}
\acro{CIR}{corotating interaction region}

\acro{CR}{Carrington rotation}

\acro{FIP}{first ionization potential}

\acro{GSE}{Geocentric Solar Ecliptic}

\acro{HCS}{Heliospheric Current Sheet}

\acro{ICME}{interplanetary coronal mass ejection}
\acro{IMF}{interplanetary magnetic field}

\acro{KS test}{Kolmogorov-Smirnov test}

\acro{L1}{1\textsuperscript{st} Earth-Sun Lagrange Point}

\acro{LTE}{local thermodynamic equilibrium} 

\acro{MEC}{Maxwell's Equation of Change}
\acro{MHD}{Magnetohydrodynamics}

\acro{PDF}{Probability Distribution Function}

\acro{PIC}{Particle-in-Cell}

\acro{SNR}{signal-to-noise ratio}
\acro{SPDF}{Space Physics Data Facility}


\acro{VDF}{velocity distribution function}

==> latex-preamble/spacecraft-instruments.tex <==
%===========================
% General Instruments
%===========================
\acro{ESA}{electrostatic analyzer}
\acro{FC}{Faraday cup}


%%===========================
%% Wind
%%===========================
%\acro{ACE}{\emph{Advanced Composition Explorer}}
\acro{SWE}{\emph{Solar Wind Experiment}}


%===========================
% ACE
%===========================
\acro{ACE}{\emph{Advanced Composition Explorer}}
\acro{SWICS}{\emph{Solar Wind Ion Composition Spectrometer}}

%===========================
% DKIST
%===========================
\acro{DKIST}{\emph{Daniel K. Inouye Solar Telescope}}


%===========================
% Helios
%===========================
\NewDocumentCommand{\Helios}{\emph{Helios}


%===========================
% IMP
%===========================
\acro{IMP}{\emph{Interplanetary Monitoring Platform}}


%===========================
% MESSENGER
%===========================
\acro{MESSENGER}{\emph{MErcury Surface Space ENvironment, GEochemistry, and Ranging}}
\acro{FIPS}{\emph{Fast Imaging Plasma Spectrometer}}


%===========================
% PSP
%===========================
\acro{PSP}{\emph{Parker Solar Probe}}
\acro{SWEAP}{\emph{Solar Wind Electrons, Alphas, and Protons}}
\acro{SPAN}{\emph{Solar Probe Analyzer}}
\acro{SPC}{\emph{Solar Probe Cup}}


\acro{\ensuremath{\mathrm{IS \! \bigodot \! IS}}}{\emph{Integrated Science Investigation of the Sun}}
\NewDocumentCommand{\ISOIS}{s}{\ac{\ensuremath{\mathrm{IS \! \bigodot \! IS}}}}


%===========================
% SolO
%===========================
\acro{SolO}{\emph{Solar Orbiter}}
\acro{HIS}{\emph{Heavy Ion Sensor}


%===========================
% Ulysses
%===========================
\acro{SWOOPS}{Solar Wind Observations Over the Poles of the Sun}


%===========================
% Wind
%===========================
\acro{MFI}{Magnetic Field Investigation}
\acro{SWE}{Solar Wind Experiment}


%===========================
% Definitions to Process
%===========================

==> latex-preamble/units_etc.tex <==
\newcommand{\nst}[1]{#1\textsuperscript{st}}
\newcommand{\nd}[1]{#1\textsuperscript{nd}}
\newcommand{\rd}[1]{#1\textsuperscript{nd}}
\newcommand{\nth}[1]{#1\textsuperscript{th}}


%==========================
%Helper commands
%==========================
\newcommand{\der}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}} 
\newcommand{\dd}[2][]{\, \mathrm{d}{ #1 } #2}









